CLIP2Protect: Protecting Facial Privacy using Text-Guided Makeup via Adversarial Latent Search

The success of deep learning based face recognition systems has given rise to serious privacy concerns due to their ability to enable unauthorized tracking of users in the digital world. Existing methods for enhancing privacy fail to generate naturalistic images that can protect facial privacy without compromising user experience. We propose a novel two-step approach for facial privacy protection that relies on finding adversarial latent codes in the low-dimensional manifold of a pretrained generative model. The first step inverts the given face image into the latent space and finetunes the generative model to achieve an accurate reconstruction of the given image from its latent code. This step produces a good initialization, aiding the generation of high-quality faces that resemble the given identity. Subsequently, user-defined makeup text prompts and identity-preserving regularization are used to guide the search for adversarial codes in the latent space. Extensive experiments demonstrate that faces generated by our approach have stronger black-box transferability with an absolute gain of 12.06% over the state-of-the-art facial privacy protection approach under the face verification task. Finally, we demonstrate the effectiveness of the proposed approach for commercial face recognition systems. Our code is available at https://github.com/fahadshamshad/Clip2Protect.

==> figtex <==
\begin{figure}[t]
\vspace{-1.4em}
\centering
\caption{\scriptsize %Proposed approach requires inversion/latent initialization for a given source image only once (52 s), and the same latent can be transferred to multiple adversarial makeup styles (19 s) (\textbf{{\color{orange}R1}},~\textbf{{\color{red}R2}}). 
We observe no artifacts for male faces (\textbf{{\color{red}R2}}). Text makeup styles for last 3 protected images from left to right are \textit{``tanned with big eyebrows" (not included in 40 styles), ``pale makeup with red lipstick"}, and \textit{``photo of a face"}, respectively. %\textit{``Tanned with big eyebrows"} is not in the 40 makeup styles used in paper, and users can use \textit{``photo of a face"} prompt if they do not want makeup (\textbf{{\color{cyan}R3}}).  Images in last 3 columns are protected.}
}
\vspace{-1em}
\includegraphics[width=0.45\textwidth]{figs/protected.pdf}
\label{fig:pipeline}
\vspace{-2.1em}
\end{figure}
